Tight Bounds for Vertex Connectivity in Dynamic Streams

We present a streaming algorithm for the vertex connectivity problem in dynamic streams with a (nearly) optimal space bound: for any $n$-vertex graph $G$ and any integer $k \geq 1$, our algorithm with high probability outputs whether or not $G$ is $k$-vertex-connected in a single pass using $\widetilde{O}(k n)$ space. Our upper bound matches the known $\Omega(k n)$ lower bound for this problem even in insertion-only streams -- which we extend to multi-pass algorithms in this paper -- and closes one of the last remaining gaps in our understanding of dynamic versus insertion-only streams. Our result is obtained via a novel analysis of the previous best dynamic streaming algorithm of Guha, McGregor, and Tench [PODS 2015] who obtained an $\widetilde{O}(k^2 n)$ space algorithm for this problem. This also gives a model-independent algorithm for computing a "certificate" of $k$-vertex-connectivity as a union of $O(k^2\log{n})$ spanning forests, each on a random subset of $O(n/k)$ vertices, which may be of independent interest.

==> OpenProblems.tex <==
% !TeX root = main.tex 
%!TEX root = main.tex

\section{Open Problems}\label{sec:open-probs}

While \Cref{thm:one-pass-con-alg} and \Cref{thm:LB-multipass} together have settled the 
complexity of the $k$-vertex connectivity problem in one pass up to poly-logarithmic factors, they 
still leave open the question of optimal space bounds (up to constant factors).
Also, obtaining optimal space bounds for multi-pass algorithms for $k$-vertex connectivity remains 
open.
We do not know tight bounds for the promised-gap $k$-vertex-connectivity problem either.

Our lower bound and those of Sun and Woodruff \cite{sun2015tight} use duplicate edges and thus 
work only on multi-graphs. 
Obtaining lower bounds for simple graphs is an open problem.
We note that our upper bound (as well as the previous ones) also hold for multi-graphs.


